Dynamics of Self-Interacting Dark Sectors

This thesis investigates the dynamics of self-interacting dark sectors in the early Universe populated through the freeze-in mechanism. The main focus is on scenarios with self-number-changing reactions of the form $2\leftrightarrow3$, and on how these interactions modify the thermal history and phenomenology of the dark sector. Several realizations are studied, including scalar theories with $\mathbb{Z}_2$ and $\mathbb{Z}_3$ symmetries, self-interacting dark matter coupled to an unstable mediator, and cannibal dark matter production during non-instantaneous reheating. The thermal evolution is obtained by solving coupled Boltzmann equations for the relevant number densities and temperatures, accounting for both freeze-in production and cannibal interactions. The resulting parameter space can be strongly constrained, effectively invisible, or potentially accessible to future searches, depending on the realization considered. Finally, the thesis studies a hidden U(1) gauge sector populated via freeze-in, where continuous energy injection can induce an inverse first-order phase transition and temporarily restore the symmetric phase, linking phase-transition dynamics and chemical equilibration in hidden sectors.

==> Chapters/backup.tex <==
Hence, the question is not if $\phi$ and $A'$ will reach local thermal equilibrium and equilibrate with each other, but when. Here we will try to quantify this more accurately. The last two interactions in Eq.~\eqref{eq:phi-A} open $s$-, $t$- and $u$-channel diagrams and ensure the regularization of the amplitude at high energies in unitary gauge. 
The squared matrix element $\vert\mathcal{M}_{2A'\to2\phi}\vert^2$ is gauge invariant. In both unitary and Feynman gauges the individual expressions involve polarization sums and are lengthy. Since we consider dark sector masses in the MeV range while production occurs at SM temperatures of order GeV, the dark photons are relativistic at production. In this limit the matrix element is approximately constant and depends only on the couplings $g$ and $\lambda$.


The dark photon distribution function obeys
%
\begin{equation}\label{eq:fBE_A}
    \left(\partial_t - H p \, \partial_p\right) f_{A'}(p,t)
    =
    C^{\bar f f \to A'}(p,t)+C^{2A'\leftrightarrow 2\phi} + C_\text{el},
\end{equation}
%
where $C_\text{el}$ encodes elastic scattering of the form $A'A'\to A'A'$. At high temperatures, we can assume that
%
\begin{equation}
	C^{\bar ff\to A'} = \Gamma_{A'\to \bar f f} \frac{m_A}{E_A}e^{-E_A/T}
\end{equation}
%
dominates. In this case, we can integrate Eq.~\eqref{eq:fBE_A}. We begin by rewriting the equation in co-moving momentum $q = a\,p$ and express the time derivative in terms of the scale factor,
%
\begin{equation}\label{eq:fA}
	\partial_a f(q,a) = \frac{C^{\bar ff\to A'}}{aH} \implies f_{A'}^{\infty}(p,a) = \frac{\Gamma_{A'\to \bar ff}m_{A'}}{H_0a_0}\int_{a_0}^{a}\,da'\frac{a^2}{y(a')} e^{-\frac{ y(a') }{a_0T_0} }\,,
\end{equation}
%
where $y(a) = \sqrt{q^2 + a^2m_{A'}^2 }$. Note that we assumed radiation domination, meaning $T = T_0a_0/a$ and $H = H_0(a_0/a)^2$. We choose $a_0  = a_\text{EWPT} = 1$, and $T_0 = T_\text{EWPT} = 150$, while for radiation domination $H_0 \simeq 3.18\times 10^{-14}\,\text{GeV}$. The
derivation for Eq.~\eqref{eq:fA} is given in the appendix ... . 


We use this solution to estimate the rate of production of $\phi$ states at high temperatures:
%
\begin{equation}\label{eq:nBE_phi_}
    \begin{split}
    	\dot n_{A} + 3Hn_A &= \Gamma_{A\to ff} n_\text{eq}^A(T)
        \\\dot n_\phi + 3Hn_\phi &= C_0^{2A'\to 2\phi} \approx \frac{\vert\mathcal{M}_{2A'\to 2\phi}\vert^2}{8\pi} \left(\int_p \frac{f_{A'}^\infty}{2E} \right)^2\,,
    \end{split}
\end{equation}
%
where we identify $\Gamma_{2A'\to 2\phi} = C_0^{2A'\to2\phi}/n_{A'}$

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.7\textwidth]{Figures/plotsCh5/prates.pdf}
	\caption{Production rate of $\Gamma_{2A'\to 2\phi}$ (blue) and the Hubble rate (orange). The upper axis denotes the temperature of the SM. At $T \simeq 100\,\text{GeV}$ we find $\Gamma_{2A\to 2\phi}=H$.}
	\label{fig:rates_H_and_Aphi}
\end{figure}

where the approximation corresponds to the relativistic limit ($\mathcal{M}_{2A'\to 2\phi}\approx\text{constant}$, $s\gg 4m_h^2,m_A^2$).
Once enough $\phi$ states are produced, elastic scattering of the form $A\phi\to A\phi$ lead to local thermal equilibrium and a shared temperature. Note that the scattering rate $\Gamma_{2A\to 2A}$, mediated by a dark Higgs, may be efficient earlier, quantitatively changing the result in~\Cref{fig:rates_H_and_Aphi}. However, qualitatively the thermalization of the dark sector still occurs at SM temperatures in the electroweak scale $T\sim 100\,\text{GeV}$, with the main conclusion unchanged.

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.7\textwidth]{Figures/plotsCh5/pfinf.pdf}
	\caption{The distribution function $p^2f_{A'}^\infty(p,a)$ at high temperatures. We choose $g = 0.3$, $v_\phi = 1\,\text{GeV}$ ($m_A = 300\,\text{MeV}$ and $m_\phi = 18.2\,\text{MeV}$) with $\epsilon = 6\times 10^{-10}$ ($\Gamma_{A\to ff} = 10^{-21}\,\text{GeV}$).}
	\label{fig:fA}
\end{figure}

%Given that $A'$ and $\phi$ achieve equilibrium very early in time when the production still UV dominted, we will assume that as soon as the $\f f\to A'$ starts, both $A'$ and $\phi$ are in local thermal equilibrium (i.e., described with a Bose-Einstein distribution with a non-vanishing chemical potential), sharing the same dark sector temperature and chemical potential.  Hence we will only track the evolution of the comoving number of particles for $\phi$ and its temperature assuming in the collision operator that the effective injection of energy is $C_0^{A'\to \bar f f}$ instead of $C_0^{2A'\to 2\phi}$, this serves as a good approximation as long as the gauge interaction is large.

